A Decentralized Sequencer and Data Availability Committee for Rollups Using Set Consensus

Blockchains face a scalability challenge due to the intrinsic throughput limitations of consensus protocols and the limitation in block sizes due to decentralization. An alternative to improve the number of transactions per second is to use Layer 2 (L2) rollups. L2s perform most computations offchain using blockchains (L1) minimally under-the-hood to guarantee correctness. A sequencer receives offchain L2 transaction requests, batches them, and commits compressed or hashed batches to L1. Hashing offers much better compression but requires a data availability committee (DAC) to translate hashes back into their corresponding batches. Current L2s consist of a centralized sequencer which receives and serializes all transactions and an optional DAC. Centralized sequencers can undesirably influence L2s evolution. We propose in this paper a fully decentralized implementation of a service that combines (1) a sequencer that posts hashes to the L1 blockchain and (2) the data availability committee that reverses the hashes. We call the resulting service a (decentralized) arranger. Our decentralized arranger is based on Set Byzantine Consensus (SBC), a service where participants can propose sets of values and consensus is reached on a subset of the union of the values proposed. We extend SBC for our fully decentralized arranger. Our main contributions are (1) a formal definition of arrangers; (2) two implementations, one with a centralized sequencer and another with a fully decentralized algorithm, with their proof of correctness; and (3) empirical evidence that our solution scales by implementing all building blocks necessary to implement a correct server.

==> OptimisticClient.tex <==
\section{Optimistic Client Implementation}~\label{app:optimistic:client}

The client presented in this section takes advantage of
knowning processes signatures.
%
Instead of contacting all data committee members, it contacts the server
processes singing the batch.
% have signed it.
%
Since there are $f+1$ different signatures, it is guaranteed that at
least one of them is from a correct server, and therefore that server
will answer with the desired batch.

\begin{algorithm}[H]
\caption{\small Optmisitc client protocol for Arranger with a
    centralized Sequencer and Data Committee.}
\label{alg:client-seqDC-opt}
\small
\begin{algorithmic}[1]
\Function{\<ArrangerApi>.\textnormal{\<add>}}{$t$}
        \State \<SequencerApi>.\<Add>(t)
    \EndFunction
    \Function{\<ArrangerApi>.\textnormal{\<translate>}}{$(id,h,\textcolor{red}{sigs(id,h)})$}
                \State $\<notContacted> \leftarrow \{ p :
                sig_p(id,h) \in sigs(id,h)\}$
        \While{not received $b$ such that $\hash(b) == h$ and
        $|\<notContacted>| > 0$}
        \State take $p$ from $\<notContacted>$
        \State \<call> $p$.\<Translate>$(h)$
        \State $\<notContacted> \leftarrow \<notContacted>
        \setminus \{p\}$

        \EndWhile
        \State \<wait> for response $b$ such that $\hash(b) == h$
        \State \<return> $b$
    \EndFunction

\end{algorithmic}
\end{algorithm}
  % \vspace{-2em}
% \input{algorithms/client-seqDC-opt}
% \input{algorithms/client-setchain-opt}
\begin{algorithm}[H]
\caption{\small Optimistic client protocol for arrangers built on
    top of setchain.}
\label{alg:client-setchain-opt}
\small
\begin{algorithmic}[1]
\Function{\<ArrangerApi>.\textnormal{\<add>}}{$t$}
        \State \<call> \<Add>$(t)$ in 1 server.
    \EndFunction
    \Function{\<ArrangerApi>.\textnormal{\<translate>}}{$(id,h,sigs(id,h))$}
        \While{not received $b$ such that $\hash(b) == h$ and there
            is a server $i$ with  $sig_i(id,h) \in sigs(id,h)$ not
            contacted yet}
            \State \<call> $i.\<Translate>(id,h)$
        \EndWhile
        \State \<wait> for response $b$ such that $\hash(b) == h$
        \State \<return> $b$
    \EndFunction

\end{algorithmic}
\end{algorithm}

% Alg.~\ref{alg:client-setchain} %and Alg.~\ref{alg:client-setchain-opt}
% provide pseudo-code for a clients, similar to the one presented
% in Section~\ref{sec:seqDC}.
% %
% From the point of view of a client, the main difference with respect
% to interacting with arrangers that consist of sequencer plus data
% committee is that in decentralized arrangers all servers implement
% operation $\<add>$.
% %
% Since $f$ servers can be Byzantine, to add a new transaction $t$,
% clients invokes $\<add>(t)$ in $f+1$ servers, ensuring that at least
% one correct server is contacted.
% %
% Here we present one option, although there are other ways of
% implementing correct clients~(see
% Appendix~\ref{app:optimistic:client})

% \input{algorithms/client-setchain}


==> algorithms/arranger-setchain.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Alg 3

\begin{figure}[b!]
\vspace{-2em}
  \begin{megaalgorithm}[H]
    \caption{\small Server implementation of decentralized \arranger extending Setchain} 
    \label{alg:arranger-setchain}
    \small
    \begin{algorithmic}[1]
        \State \textbf{extends } Setchain
        \State  \textbf{init:} $\<hashes> \leftarrow \emptyset, \<signatures> \leftarrow \emptyset, \<localsetchain>.init$
        \Function{\textnormal{\<add>}}{$t$} \label{alg:arranger-setchain-add-begin}
          \State $\<localsetchain>.\<Add>(t)$ \label{alg:arranger-setchain-add}
%          \State \<return>
        \EndFunction \label{alg:arranger-setchain-add-end}
	\Function{\textnormal{\<translate>}}{$\textit{id},h$} \label{alg:arranger-setchain-translate-begin}%\Comment{Same as in Alg.~\ref{alg:dc-member}}
        % \State \ldots
           \If{$(\<id>,\_)\notin \<hashes>$}
             \<return> \<invalidId>
           \ElsIf{$(\<id>,h)\notin \<hashes>$} \<return> \<invalidHash>
           \Else ~\<return> $\<hashes>(\<id>,h)$
           \EndIf
          \EndFunction \label{alg:arranger-setchain-translate-end}
          \Upon{$\<newepoch>(\<id>,E)$} \label{alg:arranger-setchain-upon-newepoch}
          \State $b \leftarrow \<tobatch>(E)$
          \State $h \leftarrow \hash(b)$
          \State $\<hashes> \leftarrow \<hashes> \cup \{(\<id>,h), b\}$
          \EndUpon \label{alg:arranger-setchain-upon-newepoch-end}
          \Upon{$\<added>(epoch\_signature(id,h,sig_j(\<id>,h)))$}\label{alg:arranger-setchain-upon-newsig}
          \State $\<signatures> \leftarrow \<signatures> \cup
          \{(id,h,sig_j(id,h))\}$
          \EndUpon \label{alg:arranger-setchain-upon-newsig-end}
          \Upon{$\<myturn>$} \label{alg:arranger-setchain-upon-post-begin}
          \State $id \leftarrow \<nextBatch>()$
          \State \<wait> for $f+1$ signatures
          $(id,h,sig_j(id,h))$ in \<signatures>
          \State \<logger>.\<post>$(id,h,
          \<BLSAggregate>(\bigcup_i
            sig_i(id,h)))$ \label{alg:arranger-setchain-post}
          \EndUpon \label{alg:arranger-setchain-upon-post-end}
      \end{algorithmic}
    \end{megaalgorithm}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> algorithms/client-seqDC-opt.tex <==
\begin{figure}[t!]
  \begin{algorithm}[H]
    \caption{\small Optmisitc client protocol for Arranger with a
      centralized Sequencer and Data Committee.} 
    \label{alg:client-seqDC-opt}
    \small
    \begin{algorithmic}[1]
  	\Function{\<ArrangerApi>.\<Add>}{$t$}
          \State \<SequencerApi>.\<Add>(t)
        \EndFunction
        \Function{\<ArrangerApi>.\<Translate>}{$(id,h,\textcolor{red}{sigs(id,h)})$}
                  \State $\<notContacted> \leftarrow \{ p :
                  sig_p(id,h) \in sigs(id,h)\}$
          \While{not received $b$ such that $\hash(b) == h$ and
            $|\<notContacted>| > 0$}
            \State take $p$ from $\<notContacted>$
            \State \<call> $p$.\<Translate>$(h)$
            \State $\<notContacted> \leftarrow \<notContacted>
            \setminus \{p\}$

          \EndWhile 
          \State \<wait> for response $b$ such that $\hash(b) == h$
          \State \<return> $b$
        \EndFunction
         
    \end{algorithmic}
  \end{algorithm}
  \vspace{-2em}
\end{figure}


==> algorithms/client-seqDC.tex <==
\begin{figure}[t!]
  \begin{algorithm}[H]
    \caption{\small Correct clients protocol (Sequencer + DAC).}
    \label{alg:client-seqDC}
    \small
    \begin{algorithmic}[1]
  	\Function{\<ArrangerApi>.\textnormal{\<add>}}{$t$}
          \State \<SequencerApi>.\<add>(t)
          \State \<return>
        \EndFunction
        \Function{\<ArrangerApi>.\textnormal{\<translate>}}{$\textit{id},h$}
          \ForAll{ \(p\) is a DAC member} $p$.\<translate>$(\<id>,h)$
          \EndFor
          \State \<wait> for one response $b$ with $\hash(b) == h$
          \State \<return> $b$
        \EndFunction
    \end{algorithmic}
    % \begin{algorithmic}[1]
  	% \Function{\<ArrangerApi>.\<Add>}{$t$}
    %       \State \<SequencerApi>.\<Add>(t)
    %       \State \<return>
    %     \EndFunction
    %     \Function{\<ArrangerApi>.\<Translate>}{$(id,h)$}
    %       \State $\<notContacted> \leftarrow \{ p : p \text{ is a DAC member}\}$
    %       \While{(not received $b$ with  $\hash(b) == h$) and $|\<notContacted>| > 0$}
    %         \State take $p$ from $\<notContacted>$
    %         \State \<call> $p$.\<Translate>$(h)$
    %         \State $\<notContacted> \leftarrow \<notContacted>
    %         \setminus \{p\}$
    %       \EndWhile
    %       \State \<wait> for one response $b$ with $\hash(b) == h$
    %       \State \<return> $b$
    %     \EndFunction
    % \end{algorithmic}
  \end{algorithm}
  \vspace{-2em}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> algorithms/client-setchain-opt.tex <==
\begin{figure}[t!]
  \begin{algorithm}[H]
    \caption{\small Optmisitc client protocol for Arranger built on
      top of Setchain.} 
    \label{alg:client-setchain-opt}
    \small
    \begin{algorithmic}[1]
  	\Function{\<ArrangerApi>.\<Add>}{$t$}
          \State \<call> \<Add>$(t)$ in 1 server.
        \EndFunction
        \Function{\<ArrangerApi>.\<Translate>}{$(id,h,sigs(id,h))$}
          \While{not received $b$ such that $\hash(b) == h$ and there
              is a server $i$ with  $sig_i(id,h) \in sigs(id,h)$ not
              contacted yet}
              \State \<call> $i.\<Translate>(id,h)$
          \EndWhile 
          \State \<wait> for response $b$ such that $\hash(b) == h$
          \State \<return> $b$
        \EndFunction
         
    \end{algorithmic}
  \end{algorithm}
  \vspace{-2em}
\end{figure}


==> algorithms/client-setchain.tex <==
\begin{figure}[t!]
  \begin{algorithm}[H]
    \caption{\small Correct client protocol for Arranger implemented
      on top of Setchain.}
    \label{alg:client-setchain}
    \small
    \begin{algorithmic}[1]
  	\Function{\<ArrangerApi>.\<Add>}{$t$}
          \State \<call> \<Add>$(t)$ in $f+1$  servers.
        \EndFunction
        \Function{\<ArrangerApi>.\<Translate>}{$id,h$}
          \While{not received $b$ such that $\hash(b) == h$ and there
              are servers not contacted yet}
            \State \<call> \<Translate>$(id,h)$ in a server not
            contacted before
          \EndWhile
          \State \<wait> for response $b$ such that $\hash(b) == h$
          \State \<return> $b$
        \EndFunction
         
    \end{algorithmic}
  \end{algorithm}
  \vspace{-2em}
\end{figure}


==> algorithms/dataChallenge.tex <==
\begin{figure}[!b]
  \begin{algorithm}[H]
    \caption{\small Data Availability Challenge.}
    \label{alg:dataChallenge}
    \small
    \begin{algorithmic}[1]        
    \Function{InitDataChallenge}{$\id,\merkleRoot,\sigs,\val,\sender$}\label{initDataChallenge-begin}
        % \Comment{takes the batch tag that is challenged, and the challenged staker.}
          \State \<assert> $(\id,\merkleRoot,\sigs) \in \proposedBatches$
          \State \<assert> $\val \geq \CC{data}$

          \State $\challengeId \leftarrow
          \texttt{createChallenge}(\texttt{data}, \id, \merkleRoot, \sigs)$
          \State $\challengedNode[\challengeId] \leftarrow
          (1,\texttt{hash}(\merkleRoot), \texttt{size}(\merkleRoot))$
          \State $\canBeChallenged[\challengeId] \leftarrow \emptyset$
        \EndFunction \label{initDataChallenge-end}
        \Function{PresentData}{$\challengeId, b_l, h_l,
            b_r, h_r,\sender$}
          \State \<assert> $\sender \in \texttt{stakers}(\challengeId)$
          \State $(\pos, h,  \size) \leftarrow \challengedNodes[\challengeId]$
          \State \<assert> $size > 1$
          \If {$\hash(h_l ++ h_r) \neq h$}
            \State $\texttt{removeStake}(\challengeId,\sender)$
          \Else
            \State
            $\canBeChallenged[\challengeId]
            \leftarrow (\texttt{left}(\pos), h_l, \texttt{szLeft}(size))$
            \State
            $\canBeChallenged[\challengeId]
            \leftarrow  (\texttt{right}(\pos), h_r, \texttt{szRight}(size))$
            \State $\challengedNodes[\challengeId] \leftarrow \epsilon$
            \State $\texttt{changeTurn}(\challengeId)$  
          \EndIf    
        \EndFunction
        \Function{PresentElement}{$\challengeId, e,\sender$} \label{presentElement-begin}
          \State \<assert> $\sender \in \texttt{stakers}(\challengeId)$
          \State \<assert> $n \in \challengedNodes[\challengeId]$
          \State $(\pos, h, \size) \leftarrow
          \challengedNodes[\challengeId]$
          \State \<assert> $size == 1$
          \If{$\hash(e) != h$}
             \State $\texttt{removeStake}(\challengeId,\sender)$
          \Else   
            \State $\challengedNodes[\challengeId] \leftarrow \epsilon$
          \EndIf  
        \EndFunction \label{presentElement-end} 
        \Function{ChallengeNode}{$\challengeId, \pos, \sender$}
          \State \<assert> $\challengedNode[\challengeId] \leftarrow \epsilon$
          \State \<assert> $n \in \canBeChallenged[\challengeId]$
          \State $\challengedNodes[\challengeId] = \canBeChallenged[\challengeId][n]$
          \State $\canBeChallenged[\challengeId] \leftarrow
          remove(\canBeChallenged[\challengeId], n)$
            \State $\texttt{changeTurn}(\challengeId)$
        \EndFunction
        \Function{Timeout}{$\challengeId$}
          \If{$\texttt{runoutOfTime}(\challengeId)$}
            \State $\texttt{setWinner}(\challengeId,\texttt{nextPlayer}(\challengeId))$ 
          \EndIf  
        \EndFunction   
    \end{algorithmic}
  \end{algorithm}
  \vspace{-2em}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> algorithms/integrityChallenge.tex <==
\begin{figure}
  \begin{algorithm}[H]
    \caption{\small Integrity Challenge.}
    \label{alg:integrityChallenge}
    \small
    \begin{algorithmic}[1]        
        \Function{InitIntegrityChallenge}{$\id_0,h_0,\sigs_0,e,h_e,\pos_0,\id_1,\pos_1,$
          $\staker, value, \sender$}
        % \Comment{takes the batch tag that is challenged, the element
        %   that is suspected to be duplicated, the element hash, the id
        %   of batch where the element is claimed to already appear, the
        %   position of the element in that bathch, and the challenged staker.}
          \State \<assert> $(\id_0,h_0,sigs_0) \in \proposedBatches$
          \State \<assert> $\staker \in stakers[(id_0,h_0,sigs_0)]$
          \State \<assert> $value >= cc_{integrity}$
  
          \State \<assert> $\hash(e) = h_e$ 
          \If {$\id_1 == \id_0$}
            \State $h_1 \leftarrow h_0$
          \Else
            \State \<assert> $\id_1 \in \confirmedBatches$
            \State $h_1 \leftarrow \confirmedBatches[\id_1].\hashh$
          \EndIf  
          \State $\challengeId \leftarrow
          \texttt{createChalenge}(\texttt{integrity}, \sender,
          \staker,$ $ \id_0, h_0, \sigs_0)$
          \State $\challengeState[\challengeId] \leftarrow \texttt{PathSelection}$
          \State $\Path[0][\challengeId] \leftarrow (h_e,\pos_0, h_0)$
          \State $\Path[1][\challengeId] \leftarrow (h_e,\pos_1, h_1)$
        \EndFunction
        \Function{SelectPath}{$\challengeId, \pathId, h_{\medio},\sender$}
          \State \<assert> $\challengeState[\challengeId] == \texttt{PathSelection}$
          \State \<assert> $\sender == \texttt{currentPlayer}(\challengeId)$
          \State $(h_{\bottom}, \pos_{bottom}, h_{\topp}) \leftarrow \Path[\pathId][\challengeId]$
          \State $\bottom[\challengeId] \leftarrow (\pos_{bottom}, h_{\bottom}) $
          \State $\topp[\challengeId] \leftarrow (1,h_{\topp})$ 
          \State $\medio[\challengeId] = (\texttt{midPos}(\pos_{bottom}, 1),
          h_{\medio}) $
          \State $\challengeState[\challengeId] \leftarrow \texttt{Bisection}$
          \State $\texttt{changeTurn}(\challengeId)$  
        \EndFunction
         \Function{BisectionSubpath}{$\challengeId, \topp,\sender$}
           \Comment{Same as in Alg.~\ref{alg:validityChallenge}}
         \EndFunction
         \Function{BisectionMembership}{$\challengeId, h,\sender$}
           \Comment{Same as in Alg.~\ref{alg:validityChallenge}}
         \EndFunction
        \Function{OneStepMembership}{$\challengeId, h,\sender$}
           \Comment{Same as in Alg.~\ref{alg:validityChallenge}}
         \EndFunction
        \Function{Timeout}{$\challengeId$}
           \Comment{Same as in Alg.~\ref{alg:dataChallenge}}
         \EndFunction
    \end{algorithmic}
  \end{algorithm}
  \vspace{-2em}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> algorithms/payment-client.tex <==

\begin{figure}[t!]
  \begin{algorithm}[H]
    \caption{\small API and algorithm for a client that pay for the
      translation of a hash.}
    \label{alg:sequencer}
    \small
    \begin{algorithmic}[1]

    \end{algorithmic}
  \end{algorithm}
  \vspace{-2em}
\end{figure}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> algorithms/payment-server.tex <==

\begin{figure}[t!]
  \begin{algorithm}[H]
    \caption{\small API and algorithm for server that charges for the
      translation of a hash.}
    \label{alg:sequencer}
    \small
    \begin{algorithmic}[1]
    \end{algorithmic}
  \end{algorithm}
  \vspace{-2em}
\end{figure}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> algorithms/recorder.tex <==
\begin{figure}[t!]
  \begin{algorithm}[H]
    \caption{\small Recorder.}
    \label{recorder}
    \small
    \begin{algorithmic}[1]
  	\State  \textbf{Init:} $SetchainServers$
	\hspace{2em} $L1Contract$ 
        \Function{GetEpochHashAndSignatures}{$h$}
        \State $sigs \leftarrow \emptyset$
        \While{true}
          \State $\text{pick } s \text{ from }  SetchainServers$
          \State $(S,H,\_) \leftarrow s.Get()$ \Comment{podriamos modificar la API de Setchain para que tenga algo como getEpochSigs(h) que devuelva (E,\{sign(hash(h,E))\}}
          \State $E \leftarrow H(h)$
          \State $hash\_E \leftarrow hash(<<h,E>>)$
          \State $sigs[hash\_E] \leftarrow sigs[hash\_E] \cup \{s : s = sign_i(hash\_E) \wedge \exists epoch\_signature(h,s) \in S \cup H \}$
          \If{ | sigs[hash\_E] | == f + 1}
             \State \<return> $(hash(E), sigs[hash\_E])$
          \EndIf     
         \EndWhile
         \EndFunction
     \Function{PostBatch}{}
       \State $h \leftarrow L1Contract.LastBatchNumber() + 1$
       \State $(hash,sigs) \leftarrow GetEpochHashAndSignatures(h)$
       \State \<return> $L1Contract.PostBatch(h,hash,sigs)$
       \Comment{capaz habria que juntar todas las firmas? En anytrust usan BLS.. ver bien esto!}
     \EndFunction    
    \end{algorithmic}
  \end{algorithm}
  \vspace{-2em}
\end{figure}


==> algorithms/sequencer-frontrunning.tex <==
\begin{figure}[b!]
  \begin{algorithm}[H]
    \caption{\small Centralized Sequencer that does front-running.}
    \label{alg:sequencer-frontrunning}
    \small
    \begin{algorithmic}[1]
  	\State \textbf{init: } $\<allTxs> \leftarrow \emptyset $, 
        $\<pendingTxs> \leftarrow \epsilon$,  $\<batchId>
        \leftarrow 0$ 
        \Function{add}{$t$}
          \State \ldots \Comment{Same as
            lines~\ref{seq-add}-\ref{seq-add-allTxs} in Alg.~\ref{alg:sequencer}}
          \State \textit{\<inform> Malicious client \texttt{C} about
            transaction t} \label{alg:seq-frontrunning-inform}
          \State \Return
        \EndFunction
        \Upon{\<timetopost>}
        % \When{$|pendingTxs| == \<maxSize>$ or \textit{timeout}(\(\<maxTime>\))}
          \State $b \leftarrow rearrangeTxs(\<pendingTxs>)$ \label{alg:seq-frontrunning-rearrange}
          \State \ldots \Comment{Same as
            lines~\ref{seq-when-hash-b}-\ref{seq-when-end} in Alg.~\ref{alg:sequencer}}
        \EndUpon  
        % \EndWhen
    \end{algorithmic}
  \end{algorithm}
  \vspace{-2em}
\end{figure}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> algorithms/setchain.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Alg 3
% \begin{figure}[t!]
  \begin{algorithm}[H]
  \caption{\small Server implementation of Setchain.}~\label{alg:setchain}
   \small
   \begin{algorithmic}[1]
     \State  \textbf{Init:} $\EPOCH \leftarrow 0,$
     \hspace{2em} $\HISTORY \leftarrow \emptyset,$ 
     %\State  \textbf{Init:}
     \hspace{2em}$\THESET \leftarrow \emptyset$\label{alg3:theset}
     \Function{\<Get>}{~}
        \State \<return> $(\THESET, \HISTORY,\<epoch>)$\label{alg3:get}
     \EndFunction
     \Function{\<Add>}{$e$} \label{alg3-add-begin}
        \State \<assert> $valid(e)$ and $e \notin \THESET$
        \State add element $e$ to $\<theset>$
        \State propogate $e$
        \If {$e = epoch\_signature(h,E,sign(hash(E)))$}
           \State $\<trigger>$ $\<added>(epoch\_signature(h,E,sign(hash(E))))$
        \EndIf
      \EndFunction  
      \Function{\<EpochInc>}{$h$} \label{alg3-epochinc-begin}
         \State \<assert> $h==\EPOCH +1$
         \State collaboratively compute new epoch $E$ \Comment{triggers event
           $\<newepoch>(h,E)$}
        % \State validate elements in $E$
	 \State $\THESET \leftarrow \THESET \cup E$~\label{add_theset_SBCSetDeliver}
         \State $\HISTORY \leftarrow \HISTORY \cup \{\langle h, E \rangle\}$~\label{add_history_SBCSetDeliver}
         \State $\EPOCH \leftarrow \EPOCH+1$\label{set_epoch_SBCSetDeliver} %\Comment{same as $epoch\leftarrow{}\EPOCH+1$}
         \State add $epoch\_signature(h,E,sig_i(h,hash(E)))$ to the setchain \label{alg:setchain-sign-epoch}
         \State $\<trigger>$ $\<newepoch>(h,E)$
      \EndFunction  
    \end{algorithmic}
  \end{algorithm}\vspace{-2em}
% \end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> algorithms/signatureChallenge.tex <==
\begin{figure}
  \begin{algorithm}[H]
    \caption{\small Signature Challenge.}
    \label{alg:signatureChallenge}
    \small
    \begin{algorithmic}[1]
        \Function{SignatureChallengeSize}{$\id,h,\sigs,\val,\sender$}
          \State \<assert> $(\id,h,\sigs) \in \proposedBatches$
          \State \<assert> $\val >= \CC{singature}$ 
          \If{$|sigs| < f+1$}
            \State $\texttt{removeAllStakes}(id,h,sigs,sender,\texttt{signature})$
            % \Comment{remove all stakes, discard the batch and reward
            %   the client accordingly}
           \EndIf 
         \EndFunction
         \Function{SignatureChallengeAggregation}{$\id,h,\sigs,\val,\sender$}
          \State \<assert> $(\id,h,\sigs) \in \proposedBatches$
          \State \<assert> $\val >= \CC{singature}$ 
          \State $\aggPKs \leftarrow \empty$
          \For{$i \in \sigs$}
            \State $\aggPKs \leftarrow
            \texttt{aggregatePK}(\aggPKs, \KWD{arrangerPK}[i])$
          \EndFor
          \If{$! validSignature(\aggPKs, (\id,h), \sigs)$}
            \State $\texttt{removeAllStakes}(id,h,sigs,sender,\texttt{signature})$
            % \Comment{remove all stakes, discard the batch and reward
            %   the client accordingly}
           \EndIf 
        \EndFunction
    \end{algorithmic}
  \end{algorithm}
  \vspace{-2em}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> algorithms/validityChallenge.tex <==
\begin{figure}
  \begin{algorithm}[H]
    \caption{\small Validity Challenge.}
    \label{alg:validityChallenge}
    \small
    \begin{algorithmic}[1]        
      \Function{InitValidityChallenge}{$\id,h,\sigs,e,h_e,\pos_e,h_{\medio},$ 
          $\staker,value,\sender$}
        % \Comment{takes the batch tag that is challenged, the element
        %   that is suspected to be invalid, the element hash, the hash
        %   of the medio element in the path from the leaf to the root
        %   of the merkle tree, and the challenged staker.}
           \State \<assert> $(id,h,sigs) \in \proposedBatches$
          \State \<assert> $\staker \in \stakers[(\id,h,\sigs)]$
          \State \<assert> $\value >= cc_{validity}$
           \State \<assert> $\hash(e) == h_e$ 
           \State \<assert> $\texttt{valid}(e)$
           
           \State $\challengeId \leftarrow
           \texttt{createChallenge}(\texttt{validity},
           \sender,\staker,$
           $\id, h, \sigs)$
           \State $challengeState[\challengeId] \leftarrow \texttt{Bisection}$
           \State $\bottom[\challengeId] \leftarrow (\pos_e, h_e)$
           \State $\topp[\challengeId] \leftarrow (1, h)$
           \State $\medio[\challengeId] \leftarrow (\texttt{midPos}(1, \pos_e), h_{\medio})$
         \EndFunction
         \Function{BisectionSubpath}{$\challengeId, \topp,\sender$}
           \State \<assert> $\challengeState[\challengeId] == \texttt{Bisection}$
           \State \<assert> $\sender == \texttt{currentPlayer}(\challengeId)$
           \If {$\topp$}
             \State $\bottom[\challengeId] \leftarrow \medio[\challengeId]$
           \Else
             \State $\topp[\challengeId] \leftarrow \medio[\challengeId]$ 
           \EndIf
           \If {$\texttt{dist}(\bottom[\challengeId].\pos, \topp[\challengeId].\pos) ==
               1$}
             \State $\challengeState[\challengeId] \leftarrow
             \texttt{OneStep}$
           \EndIf  
           \State $\texttt{changeTurn}(\challengeId)$  
         \EndFunction
         \Function{BisectionMembership}{$\challengeId, h,\sender$}
           \State \<assert> $\challengeState[\challengeId] == \texttt{Bisection}$
           \State \<assert> $\sender == \texttt{currentPlayer}(\challengeId)$
           \State $\medio[\challengeId] =
           (\texttt{midPos}(\topp[\challengeId].\pos, \bottom[\challengeId].\pos), h)$
         \EndFunction
         \Function{OneStepMembership}{$\challengeId, h,\sender$}
           \State \<assert> $\challengeState[\challengeId] == \texttt{OneStep}$
           \State \<assert> $\sender == \texttt{currentPlayer}(\challengeId)$
           \State $c \leftarrow \texttt{concatenate}(\bottom[\challengeId],
           h)$
           \If{$\hash(c) == \topp[challengeId].\hashh$}
             \State $\texttt{setWinner}(\challengeId,\texttt{currentPlayer}(\challengeId))$ 
           \Else
             \State $\texttt{setWinner}(\challengeId,\texttt{nextPlayer}(\challengeId))$
           \EndIf  
         \EndFunction
         \Function{Timeout}{$\challengeId$}
           \Comment{Same as in Alg.~\ref{alg:dataChallenge}}
         \EndFunction   
    \end{algorithmic}
  \end{algorithm}
  \vspace{-2em}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> figures/latex/preamble.tex <==
\pdfobjcompresslevel0

\usepackage[T1]{fontenc}
\usepackage[tt=false, type1=true]{libertine} 
\usepackage[varqu]{zi4}
\usepackage[libertine]{newtxmath}
\usepackage{amssymb}
\usepackage{algorithm}
\usepackage{algpseudocode}


